Nonreversible MCMC from conditional invertible transforms: a complete recipe with convergence guarantees

Markov Chain Monte Carlo (MCMC) is a class of algorithms to sample complex and high-dimensional probability distributions. The Metropolis-Hastings (MH) algorithm, the workhorse of MCMC, provides a simple recipe to construct reversible Markov kernels. Reversibility is a tractable property that implies a less tractable but essential property here, invariance. Reversibility is however not necessarily desirable when considering performance. This has prompted recent interest in designing kernels breaking this property. At the same time, an active stream of research has focused on the design of novel versions of the MH kernel, some nonreversible, relying on the use of complex invertible deterministic transforms. While standard implementations of the MH kernel are well understood, the aforementioned developments have not received the same systematic treatment to ensure their validity. This paper fills the gap by developing general tools to ensure that a class of nonreversible Markov kernels, possibly relying on complex transforms, has the desired invariance property and leads to convergent algorithms. This leads to a set of simple and practically verifiable conditions.

==> lifted.tex <==
% !TEX root = main-t.tex

\subsection{Lifted kernels}
In this section, we apply the results of \Cref{sec:mu-s-reversibility}
to lifted kernels introduced in~\cite{diaconis:holmes:neal:2000,chen:lovasz:pak:1999,turitsyn:2011,michel:2016}. As
above, let $\target$ be a target probability density on $\rset^d$
\wrt~the Lebesgue measure. We extend the state space with a direction,
\ie\ we consider $\msz = \rset^d \times \msv$ with $\msv = \{-1,1\}$
and the extended target distribution
$\exttarget = \target \otimes [\{\updelta_{-1} +
\updelta_{1}\}/2]$. In this scenario the involution is
$\invf(x,v) = (x,-v)$.

\paragraph{Proposal with densities.} Let $q_{-1}(x,\cdot),q_{1}(x,\cdot)$  be two
transition densities \wrt\ the Lebesgue
measure on $\rset^d$. Consider a proposal kernel $Q((x,v), \rmd(y,w))$ with density $q((x,v), (y,w)) $ with
respect to $\Leb_d(\rmd y) \otimes \{\updelta_{-1}(\rmd w) + \updelta_{1}(\rmd w)\}$ given by
{\small\begin{equation}
\label{eq:lifted_density}
q\bigl((x,v), (y, w)\bigr)= \bigl\{\probav \indi{v}(w) +(1-\probav) \indi{-v}(w)\bigr\}  q_w(x,y),
\end{equation}}

\vspace{-0.7cm}
\noindent
where $\probav \in \ooint{0,1}$. In words, starting from $(x,v)$, we either ``keep" $w=v$ with probability $\probav$ or
``flip" $w=-v$ the direction otherwise, and then propose a
candidate $y$ according to $q_{w}(x,\cdot)$. In the original implementation of the lifting procedure \cite{turitsyn:2011}, $\probav$ is set to $1$; taking $\probav <1$ simply prevents the algorithm from getting ``stuck" in one direction which could impede convergence of the algorithm.

From~\eqref{eq:generalized-MH} and~\eqref{eq:alpha_density}, the
acceptance ratio $\alpha$ writes, for
$q_w(x,y)\target(x) \neq 0$, see \Cref{sec:proof:alpha_lifted},
% {\small\begin{multline}
% \label{eq:alpha_lifted}
% \alpha((x,v),(y,w))= \accfun\left(\frac{q_{-v}(y,x) \target(y)}{q_v(x,y)\target(x)}\right) \indi{v}(w) \\
% +\accfun\left(\frac{q_{v}(y,x) \target(y)}{q_{-v}(x,y)\target(x)}\right) \indi{v}(-w) \eqsp.
% \end{multline}}
%{\small
\begin{equation}
\label{eq:alpha_lifted}
\alpha\bigl((x,v),(y,w)\bigr)= \accfun\left(\frac{q_{-w}(y,x) \target(y)}{q_w(x,y)\target(x)}\right) \eqsp,
\end{equation}
%}
%
%\vspace{-0.5cm}
%\noindent
and $\alpha\bigl((x,v),(y,w)\bigr) = 1$ otherwise, where $\accfun$ satisfies
\eqref{eq:prop_accfun}. The GMH kernel is given by
\eqref{eq:kernel-with-mass} with $a(z)=0$ and
$b(z)= 1 - Q_{\alpha}\bigl((x,v),\Zset\bigr)$. Note that if the proposal move is
rejected, then the direction is automatically flipped.

In the case
$q_{-1} = q_{1}$, then the acceptance probability $\alpha$ \eqref{eq:alpha_lifted} does not
depend on $v,w$ and the GMH kernel~\eqref{eq:kernel-with-mass} can be
marginalized \wrt~$v$ yielding the $\pi_0$-reversible MH
algorithm of proposal density $q_1$. Since $\probav \in \ooint{0,1}$, the expression for $q$ in
\eqref{eq:lifted_density} implies the following result.
\begin{proposition}
  \label{propo:lifted_density}
Assume that  for any
$y \in \rset^d$, $\pi_0(y) >0$ implies $q_{-1}(x,y) >0$ and
$q_1(x,y) >0$, for all $x\in\rset^d$.  Then the conditions of
\Cref{theo:irred_and_co} hold, and the  GMH kernel~\eqref{eq:kernel-with-mass} is
ergodic.
\end{proposition}


Similarly to \Cref{sec:gener-hamilt-dynam}, the proposal densities $q_{v}(x,\cdot)$ are often associated to $\rmc^1$-diffeomorphisms $G_{v,x}\colon p\mapsto G_{v,x}(p)$. From a state $X_k$, we sample $P_{k+1}$ from $\varphi$ positive density on $\rset^{d}$ and set $Y_{k+1} = G_{V_k, X_k}(P_{k+1})$. 
%deterministic transforms $G_v\colon \rset^d\times \rset^d\to \rset^d$, for $v \in \msv$, satisfying  for any $x\in \rset^d, v\in \msv$, that $p\mapsto \tilde{G}_{v,x}(p) = G_v(x,p)$ is a $\rmc^1$-diffeomorphism, which can be established as in Subsection \ref{sec:gener-hamilt-dynam}. 
In this case,  
\begin{equation}
  \label{eq:def_q_v}
  q_v(x,y) = \varphi\bigl(G_{v,x}^{-1}(y)\bigr) \Jac_{G_{v,x}^{-1}}(y)  \eqsp.
\end{equation}
%using the change of variable $y = G_{v,x}(p)$.
%$Q_vf(x)=\int f\bigl(G_{v,x}(p)\bigr) \varphi(p) \rmd p$.

We illustrate the construction above with two examples of mappings $G$ satisfying the conditions we consider.
\begin{example}[(MALA-cIT) lifted kernel]
  Assume that $\pi_0$ is positive and continuously differentiable. For $x\in\rset^d$, we define two transforms $G_{1,x}, G_{-1,x}$. For $G_{1,x}$, we set
\begin{equation}
G_{1,x}\colon p\mapsto x + \gamma \nabla \log\pi(x) + \sqrt{2\gamma} p\eqsp,
\end{equation}
which corresponds to the proposal of the Metropolis Adjusted Langevin Algorithm (MALA).
In particular, for any $x\in\rset^d$, the transformation $G_{1,x}$ is a $\rmc^1$-diffeomorphism, with $\Jac_{G_{1,x}}(p) =  (2 \gamma)^{d/2}$ and 
\begin{equation}
G_{1,x}^{-1}(y) = \{y-x-\gamma \nabla \log \pi (x)\}/\sqrt{2 \gamma} \eqsp.
\end{equation}
\label{example:cIT}
For $G_{-1,x}$ we consider conditional invertible transforms~\cite{ardizzone:2019}
\begin{equation}
%  \label{eq:3}
  G_{-1,x}(p) = \LG_{K,x}\circ\dots\circ \LG_{1,x}(p) \eqsp,
\end{equation}
where for $i \in \{1,\ldots,K\}$, $\LG_{i,x}$ splits its input
into two parts $(p_{i,1},p_{i,2})\in\rset^{d_{i,1}}\times\rset^{d-d_{i,1}}$ and applies affine transformations between them
\begin{equation}
\begin{aligned}
p_{i+1,1}& = p_{i,1} \odot \exp\bigl(R_{i,1}(p_{i,2},x)\bigr) + M_{i,1}(p_{i,2},x) \eqsp,\\
p_{i+1,2}& = p_{i,2} \odot \exp\bigl(R_{i,2}(p_{i+1,1},x)\bigr) + M_{i,2}(p_{i+1,1},x) \eqsp.
\end{aligned}
\end{equation}
Here $R_{i,1},M_{i,1}$ (resp. $R_{i,2},M_{i,2}$) are any functions from $\rset^{d_{i,1}}$ (resp. $\rset^{d-d_{i,1}}$) to $\rset^d$.
This structure is an extension of the affine coupling block
architecture suggested in~\cite{dinh:2016}. Note that for any
$i \in \{1,\ldots,K\}$, $\LG_{i,x}$ is a $\rmC^1$-diffeomorphism on
$\rset^d$ of Jacobian determinant given by
$\Jac_{\LG_{i,x}}(p) = \exp\bigl(R_{i,1}(p_2,x)+R_{i,2}(p_1',x)\bigr)$. Therefore,
$G_{-1,x}$ is a
$\rmC^1$-diffeomorphism with Jacobian determinant which can be explicitly computed.~\eqref{eq:def_q_v} gives a nonreversible MH algorithm with convergence guarantees provided by \Cref{propo:lifted_density};
see details in \Cref{subsec:cIT_implementation}.

%Setting $G_1 = G_{\MALA}$ and $G_{-1} = G_{\cIT}$ in
%Thus,~\eqref{eq:def_q_v} gives a nonreversible MH algorithm with convergence guarantees provided by \Cref{propo:lifted_density}.
\end{example}

A specific case corresponds to the choice
\begin{equation}
  \label{eq:def_forward_back_G_transf}
  G_{v,x}(p) = \projq \circ \transflif^v(x,p) \eqsp,
\end{equation}
where $\transflif$
is a $\rmc^1$-diffeomorphism on $\rset^{2d}$.
We establish in the following result an
alternative expression for $\alpha$ using~\eqref{eq:alpha_lifted} and~\eqref{eq:def_q_v}, which relies on $\transflif^v$ and
$\Jac_{\transflif^v}$ and for which $\Jac_{G_{v,x}}$ is not required anymore (see \Cref{sec:proof:altern_accfun}).
\begin{lemma}
  \label{lem:altern_accfun}
  Assume that, for any $(x,v) \in \Zset$, the mapping $G_{v,x}$ is a
$\rmc^1$-diffeomorphism on $\rset^d$. Then, for any $x,y \in \rset^d$, $v,w \in \msv$, the acceptance ratio $\alpha$ defined in \eqref{eq:alpha_lifted}% corresponding to $q_v$ defined by
  % \eqref{eq:def_q_v}
  is given by
%{\small 
\begin{equation}
%    &\alpha(x,v;y,w)
    % = \phi\left(\frac{\Jac_{G^{-1}_{-v,y}}(x) \varphi(G^{-1}_{-v,y}(x)) \pi(y)}{\Jac_{G^{-1}_{v,x}}(y) \varphi(G^{-1}_{v,x}(y))\pi(x)}\right) \indi{v}(w)
   % \\
 \accfun\left(\frac{ \mu\Bigl(\transflif^{w}\bigl(x, G^{-1}_{w,x}(y)\bigr)\Bigr)}{\mu\bigl(x, G^{-1}_{w,x}(y)\bigr)}\Jac_{\transflif^w}\bigl(x, G^{-1}_{w,x}(y)\bigr)\right)  \eqsp,
\end{equation}%}
where $\mu(x,p) = \pi_0(x)\varphi(p)$.
\end{lemma}
This result is of practical interest because in many cases, the computation of $\Jac_{\transflif^v}(x,p)$ is much simpler than that of $\Jac_{G_{v,x}}(p)$. As an example, if $\transflif$ is the generalized HMC transform $\transflif= \LF_m\circ\dots\circ\LF_1$ where $\LF_i$ is defined in \eqref{eq:definition-nice-flow}, $\Jac_{\transflif^v}(x,p)=1$ while $\Jac_{G_{v,x}}(p)$ has no simple closed-form expression.
%% Here we can't write the diffeomorphism  $\tidle{G}_{v,x}$ ony for generalized MALA in practice in experiments -> write it in previous section ?
% \begin{example}
% Consider real-NVP \cite{dinh:krueger:bengio:2014} like transitions for our MCMC algorithm.
% This framework could include in particular the Generalized Hamiltonian Monte Carlo algorithm presented in \citep{levy:hoffman:sohl-dickstein:2017,gu:sun:2020}.
% Consider families of transformations $\{s_k\}_{k=1}^{K}$, $\{t_k\}_{k=1}^K$ and $\{M_k\}_{k=1}^K$, $\{N_k\}_{k=1}^K$.
% We write the transitions as follows $T_i (x_i, p_i) = (x_{i+1}, p_{i+1})$, where
% \begin{equation}
% \begin{cases}
% p_{i+1/2} &= \exp\{h s_i(x_i)\} \odot p_i + h M_i(x_i) \\
% x_{i+1} &= x_i + h p_{i+ 1/2} \\
% p_{i+1} &= \exp\{h t_i(x_{i+1})\} \odot p_{i+1/2} + h N_{i}(x_{i+1})
% \end{cases}.
% \end{equation}
% The inverse of this mapping is easily obtained \suppl.
% \end{example}
\paragraph{Deterministic proposals.}

Using a $\rmC^1$-diffeomorphism $\Psi$ on $\rset^{2d}$, we may also consider deterministic moves like in \Cref{sec:gener-hamilt-dynam}. Consider the extended state space
  $\msz = \rset^{2d} \times \msv$, the target distribution
  $\pi = \pi_0 \otimes \varphi \otimes
  [\{\updelta_{-1}+\updelta_{1}\}/2]$, where $\varphi$ is a symmetric
  density \wrt~$\Leb_d$, and the involution  $\invol(x,p,v) =   (x,p,-v)$.
Define
$\transflifdet\bigl(x,p,v\bigr) = \bigl(\transflif^v(x,p),v\bigr)$. Then, it is immediate to see that
$\invol \circ \transflifdet \circ \invol =
\transflifdet^{-1}$. We consider the deterministic proposal
kernel
\begin{equation}
  Q\bigl((x,p,v),\rmd(y,q,w)\bigr) = \updelta_{\transflif^v(x,p)}(\rmd (y,q)) \updelta_{v}(\rmd w) \eqsp.
\end{equation}
In the case, the
acceptance ratio \eqref{eq:generalized-MH-deterministic}
reads for $x,p\in\rset^d$,  $v \in \msv$ satisfying $ \pi_0(x)\varphi(p) > 0$% (y,q,w)= (\transflif^v(x,p),v)$
%{\small{
\begin{equation}
\label{eq:acceptance-probability-determinist-lif}
\bar{\alpha}(x,p,v) = \accfun\left( \mu\bigl(\transflif^v(x,p)\bigr) \Jac_{\transflif^v}(x,p)/{\mu(x,p)} \right) \eqsp,
\end{equation}
%}}
%
%\vspace{-0.6cm}
%\noindent
and is equal to $1$ if $\mu(x,p)=0$, where $\mu(x,p)= \pi_0(x)\varphi(p)$; see \Cref{subsec:proof_lifted_deterministic}.

\begin{example}[L2HMC]
  \label{ex:l2hmc}
  Assume that $\pi_0$ is positive and continuously differentiable.
  Using the framework depicted above, we show how the L2HMC algorithm~\cite{levy:hoffman:sohl-dickstein:2017} (Learning To Hamiltonian Monte Carlo) can be turned into a
  nonreversible MCMC method by considering the
  map
\begin{equation}
  \label{eq:def_lDhmc}
  \transflif(x,p) = G_{K}\circ\dots\circ G_{1}(x,p) \eqsp,
\end{equation}
where $G_i = H_{i} \circ F_{i} \circ H_{i-1/2}$ with, for $\delta>0$, 
\begin{enumerate}[wide, labelwidth=!, labelindent=0pt,label=$\bullet$,noitemsep,nolistsep]
\item for $j \in \{i,i-1/2\}$, $H_j(x,p)=(x, H_{j,x}(p))$ with
{\small  
  \begin{multline}
    H_{j,x}(p) =p \odot \exp\left(\delta R_{j}^H(x)\right)\\ +\delta
  \bigl[\nabla \log \pi_0(x) \odot \exp\left(\delta R_{j}^H(x)\right)+
  M_{j}^H(x)\bigr]\eqsp.
  \end{multline}
  }
   Note that $H_j$ is a $\rmc^1$-diffeomorphism on
  $\rset^{2d}$ of Jacobian $\Jac_{H_j}(x,p)=\exp\left(\delta R_{j}^H(x)\right)$.
\item $F_i(x,p) = \bigl(F_{i,p}(x),p\bigr)$, where
  $F_{i,p}$ splits its input
into two parts $x_1,x_2$ and applies affine transformations
{\small\begin{equation}
\begin{aligned}
x_1'& = x_1 \odot \exp\bigl(\delta R^F_{i,1}(x_2,p)\bigr) + \delta M^F_{i,1}(x_2,p) \eqsp, \\
x_2'& = x_2 \odot \exp\bigl(\delta R^F_{i,2}(x_1',p)\bigr) + \delta M^F_{i,2}(x_1',p) \eqsp.
\end{aligned}
\end{equation}}
Clearly, $F_{i}$ is a $\rmc^1$-diffeomorphism on $\rset^{2d}$ with $\Jac_{F_i}(x,p) =\exp\bigl(\delta R_{i,1}^F(x_2,p)+\delta R_{i,2}^F(x_1',p)\bigr)$.
\end{enumerate}
Then, $\transflif$ defined by~\eqref{eq:def_lDhmc} is a
$\rmC^1$-diffeomorphism whose Jacobian can be recursively computed. Then, the kernel $P(x,p,w),\rmd (y,q,w))$ given by
\begin{multline}
 \bar{\alpha}(x,p,v)\updelta_{\transflif^v(x,p)}(\rmd (y,q)) \updelta_{v}(\rmd w) \\
+ (1- \bar{\alpha}(x,p,v))\updelta_{(x,p,-v)}(\rmd (y,q,w))
\end{multline}
where $\bar{\alpha}$ is defined in \eqref{eq:acceptance-probability-determinist-lif} is $(\pi, S)$-reversible. This kernel should be combined with (possibly partial) refreshment steps as discussed in \Cref{sec:gener-hamilt-dynam}; see \Cref{subsec:l2hmc_implem} for details.
\end{example}

% Note that compared to its original definition, the formulation provided by \Cref{lem:altern_accfun} only relies on $\transflif^v$ and  $\Jac_{\transflif^v}$.
% and show that % for any $
% \begin{align}
%     \transflif:&\rset^d\times\rset^d \to \rset^d\times\rset^d
%     \\
%     &(x,p)\mapsto \transflif(x,p)
% \end{align}
% and the mappings $G_v$ defined by $G_v(x,p) = \sigma_x \circ \transflif^v(x,p)$ with $\sigma_x(x,p) = x$ for $(x,p)\in \rset^{2d}$
% Thus, from the mappings $G_v$, we can obtain a $(\mu, \Sigma)$-reversible kernel, with the acceptance function $\alpha$
% \begin{equation}
% \alpha(x,v;y,w) = \phi\left(\frac{\Jac_{\tilde{G}^{-1}_{-v,y}}(x) \varphi(\tilde{G}^{-1}_{-v,y}(x)) \pi(y)}{\Jac_{\tilde{G}^{-1}_{v,x}}(y) \varphi(\tilde{G}^{-1}_{v,x}(y))\pi(x)}\right) \indi{v}(w)
% \end{equation}

% Another special case of this representation is when we consider a $\rmc^1$ diffeomorphism
% \begin{align}
%     \transflif:&\rset^d\times\rset^d \to \rset^d\times\rset^d
%     \\
%     &(x,p)\mapsto \transflif(x,p)
% \end{align}
% and the mappings $G_v$ defined by $G_v(x,p) = \sigma_x \circ \transflif^v(x,p)$ with $\sigma_x(x,p) = x$ for $(x,p)\in \rset^{2d}$ and $\transflif^{-1}$ is the inverse of $\transflif$.
% If the same assumption holds for $G_v$, then we can write the function \begin{align}
%    &\alpha(x,v;y,w) = \phi\left(\frac{\Jac_{\tilde{G}^{-1}_{-v,y}}(x) \varphi(\tilde{G}^{-1}_{-v,y}(x)) \pi(y)}{\Jac_{\tilde{G}^{-1}_{v,x}}(y) \varphi(\tilde{G}^{-1}_{v,x}(y))\pi(x)}\right) \indi{v}(w)
%    \\
%    & =\phi\left(\frac{\pi\otimes\varphi(\transflif^v(x, \tilde{G}^{-1}_{-v,y}(x))}{\pi\otimes\varphi(x, \tilde{G}^{-1}_{v,x}(y))}\Jac_{\transflif^v}(x, \tilde{G}^{-1}_{v,x}(y))\right) \indi{v}(w)
% \end{align}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main-t"
%%% End:


==> menage.tex <==
% <<<<<<< HEAD
% We construct a Markov kernel which generalized the HMC construction (see \cite{neal:2011,sohl2014hamiltonian}. and might also be seen as a special case of NICE MCMC methods \cite{song2017nice,neklyudov:welling:vetrov:2020}. The objective is to sample $\pi_0(\rmd x)= \pi_0(x) \Leb(\rmd x)$ where  $\pi_0: \rset^d \to \rset_+$ is a pdf \wrt\ the Lebesgue measure $\Leb$. We use a data augmentation approach which consists in adding a "momentum" random variable with a symmetric pdf $\varphi$ on $\rset^d$, \eg~$\phi(-p) = \phi(p)$. More precisely, on the extended state space $\Zset= \rset^{2d}$, we consider the extended target density defined by $\pi(x,p)= \pi_0(x) \varphi(p)$. The involution is taken to be $\invol(x,p)= (x,-p)$. By construction, $\pi(\invol(x,p))= \pi(x,p)$.

% Based on the results of the previous section, we first show how to construct a  $(\pi,\involk)$-reversible on $\rset^{2d}$ using modified leap-frog integrators.  Let $h >0$, $m \in \nset$ and $\{\transfm_i,\transfn_i\}_{i=1}^m$ be $\rmc^1$ functions on $ \rset^{d}$. The NICE transform we consider is  defined by composing $m$ elementary mappings $\transfdet(x,p) = \transfdet_{k} \circ \cdots \circ \transfdet_1(x,p)$, given, for any
% $i \in\{1,\ldots,m\}$, by $(x_{i+1},p_{i+1}) = \transfdet_{i}(x_i,p_i)$ where
% \small{
%=======


==> nice_p.tex <==
\subsection{Generalized Hamiltonian Dynamics}

We first consider a generalization of the Hamiltonian Monte Carlo algorithm (see \cite{neal:2011,sohl2014hamiltonian}. These methods might also be seen as a special case of NICE MCMC methods \cite{song2017nice,neklyudov:welling:vetrov:2020} where NICE stands for Non-linear Independent Components Estimation. The objective is to sample a distribution $\pi_0(\rmd x)= \pi_0(x) \Leb(\rmd x)$ on $\rset^d$ with density $\pi_0$ \wrt\ the Lebesgue measure $\Leb$. We use a data augmentation approach which consists in adding a "momentum" random variable with stationary distribution admitting a symmetric density $\varphi$ on $\rset^d$ \wrt $\,\Leb$, \eg~$\varphi(-p) = \varphi(p)$. More precisely, we consider the extended state space $\Zset= \rset^{2d}$, the extended target density defined by $\pi(x,p)= \pi_0(x) \varphi(p)$ and the involution $\invol(x,p)= (x,-p)$.  We let $\big(Z_i=(X_i,V_i)\big)_{i \in \nset}$ be the corresponding Markov chain on $\rset^{2d}$. It is easily seen that $\pi(\invol(x,p))= \pi(x,p)$ and $\pushf{s} (\Leb \otimes \Leb) = \Leb \otimes \Leb$.

Based on the results of the previous section, we first show how to construct a  $(\pi,\involk)$-reversible Markov kernel on $\rset^{2d}$ using modified leap-frog integrators.  Let $m \in \nset$ and $\{\transfm_i,\transfn_i\}_{i=1}^m$ be $\rmc^1$ functions on $ \rset^{d}$. The NICE transform we consider is  defined by composing $m$ elementary mappings $\transfdet(x,p) = \transfdet_{k} \circ \cdots \circ \transfdet_1(x,p)$, given, for any
$i \in\{1,\ldots,m\}$, by $(x_{i+1},p_{i+1}) = \transfdet_{i}(x_i,p_i)$ where for $h>0$
{\small{
\begin{equation}
  \label{eq:definition-nice-flow}
  \begin{cases}
    p_{i+1/2} &= p_{i} + h \transfm_i(x_i) \\
    x_{i+1} &= x_i +h p_{i+1/2} \\
    p_{i+1} &= p_{i+1/2} + h\transfn_i(x_{i+1}) \eqsp.
  \end{cases}
\end{equation}
}
}

\vspace{-0.5cm}
\noindent 
It is easily seen that, for any $i \in \{1,\ldots,m\}$, $\transfdet_{i}$ is $\rmc^1$ diffeomorphism on $\rset^{2d}$ to $\rset^{2d}$ and its inverse satisfies $\transfdet_{i}^{-1}= \invol \circ \transfdet_i \circ \invol$.
Note also that  each transformation $\transfdet_{i}$ is the composition of 3 shear transforms $\suppl$ which implies that  $\Jac_{\transfdet_i}(x,p)= 1$ where $\Jac_f$ denotes the Jacobian of $f$.

Following the method outlined in \Cref{sec:mu-s-reversibility}, we first identify the dominating measure $\lambda$ (see \eqref{eq:definition-k-lambda})  which is easily shown to have a density \wrt\ $\Leb_{2d}$ given by \suppl\ :
\begin{equation}
\label{eq:definition-lambda}
\lambda(\rmd (x,p)) = \{ \pi (x,p) + \pi \circ \transfdet(x,p) \} \Leb_{2d}(\rmd (x,p))
\end{equation}
The density $k$ is respectively defined as
\begin{equation}
\label{eq:definition-density-nice}
k(x,p)= \frac{\rmd \pi}{\rmd \lambda}(x,p)= \frac{\pi(x,p)}{\pi (x,p) + \pi \circ \transfdet(x,p)} \eqsp.
\end{equation}
Since $\pi \circ \invol= \pi$ and $\transfdet \circ \invol \circ \transfdet= \invol$, we  obtain similarly
\begin{equation}
\label{eq:definition-density-nice-transformed}
k( \invol \circ \transfdet(x,p))= \frac{\pi(\transfdet(x,p))}{\pi(x,p) + \pi(\transfdet(x,p))}
\end{equation}
Hence, the acceptance ratio is given by
\begin{equation}
\label{eq:generalized-MH-deterministic-nice}
\bar{\alpha}(x,p)= \accfun\left( \frac{\pi \circ \transfdet(x,p)}{\pi(x,p)} \right)
\end{equation}
if $\pi(x,p) >0$ and is equal to 1 otherwise.

Such kernels are deterministic an therefore (most likely) not ergodic. Similar to Hamiltonian MC, a possible solution is to refresh the momentum between two successive NICE moves. For simplicity, we consider in this paper only a "full refresh", which amounts to draw a new value of the momentum at each iteration from $\varphi$.
Combining the refresh step with the NICE move and marginalizing \wrt\ the momentum random variable, we define
a Markov kernel on $\rset^d$
{\small \begin{equation}
\label{eq:marginal-NICE-kernel}
P(x,\rmd y)= Q_\alpha(x,\rmd y) + \{1- \bar{\alpha}(x) \} \updelta_{x}(\rmd y)
\end{equation}
}

\vspace{-0.5cm}
\noindent
where $\bar{\alpha}(x) = \int \bar{\alpha}(x,p) \varphi(p) \rmd p$ is the average rejection rate and
$Q_\alpha(x,\rmd y)= \int \bar{\alpha}(x,p) \varphi(p) \updelta_{\transfdet_1(x,p)}(\rmd y) \rmd p$ with
$\transfdet_1(x,p)= \projq \circ \transfdet(x,p)$ where $\projq(x,p)= x$.

{\color{blue} Such Markov kernels are purely deterministic and therefore (most likely) not
ergodic. A standard approach to address this issue, used in the context of HMC algorithms, is to refresh the
momentum between two successive NICE moves according to a Markov transition 
preserving the distribution $\varphi \times \Leb$. A particular choice consists of sampling the velocity afresh from $\varphi \times \Leb$ before applying the kernel \eqref{eq:kernel-with-mass}. In this case one can check that $(X_i)_{i \in \nset}$ is a Markov chain on $\rset^d$ of kernel, obtained by marginalisation of \eqref{eq:kernel-with-mass} \wrt\ the momentum distribution,
 \begin{equation}
\label{eq:marginal-NICE-kernel}
K(x,\rmd y)= K_\alpha(x,\rmd y) + \{1- K_{\alpha}(x,\rset^d) \} \updelta_{x}(\rmd y) \eqsp,
\end{equation}
where  $K_\alpha(x,\rmd y)= \int \bar{\alpha}(x,p) \varphi(p) \updelta_{\transfdet_1(x,p)}(\rmd y) \rmd p$ with
$\transfdet_1(x,p)= \projq \circ \transfdet(x,p)$, $\projq(x,p)= x$.
In this scenario $(X_i)_{i \in \nset}$ is time-reversible (see e.g. \cite{duane:1987}), which has the disadvantage of loosing the potentially advantageous persistency features of $P$. It is possible to recover persistency by considering the mixture of kernels $L:=\omega K \otimes (\varphi \times \Leb) + (1-\omega) P$ for $\omega \in [0,1]$. In what follows we establish $\Leb-$irreducibility of $K$, which immediately implies $\Leb\otimes\Leb-$irreducibility of $L$.
}

Assume now that for any $x \in \rset^d$, $p \mapsto G_x(p) = \transfdet_1(x,p)$ is a diffeomorphism on $\rset^d$.
<<<<<<< HEAD
For the GMH proposal \eqref{eq:definition-nice-flow}, this assumption is satisfied provided that for any $i \{1,\dots, m\}$, $M_i$ and $N_i$ are $\mathrm{L}$-Lipschitz,  differentiable and \tcr{$h \leq xxx$}.
In such case, $Q_\alpha(x,\rmd y)= \alpha(x,y) q(x,y) \Leb_d(\rmd y)$ with
=======
For the GMH proposal \eqref{eq:definition-nice-flow}, this assumption is satisfied provided that for any $i \in  \{1,\dots, m\}$, $M_i$ and $N_i$ are $\mathrm{L}$-Lipschitz and  $h \leq c_0/[\mathrm{L}^{1 / 2}m]$, 
 where $c_0\in\rset^{+}$ is defined in supplementary material, see \Cref{SPsec:ergodicity} .
In this scenario, $K_\alpha(x,\rmd y)= \alpha(x,y) q(x,y) \Leb(\rmd y)$ with \christophe{I wonder if this is not what should be put forward as a clear separate statement}
>>>>>>> 812d27c8fa67b85e4bad7a49278eae8d39be7436
{\small{
\begin{align}
\label{eq:acceptance-NICE}
\alpha(x,y) &= \accfun\left(\frac{\pi_0(y) \varphi(H_x(G_x^{-1}(y)))}{\pi_0(x) \varphi(G_x^{-1}(y))} \right) \, \\
\label{eq:density-NICE}
q(x,y) &= \varphi(G_x^{-1}(y)) \Jac_{G_x^{-1}}(y) \eqsp,
\end{align}
}}
<<<<<<< HEAD
with $H_x(p)= \projp \circ \transfdet(x,p)$ and $\projp(x,p)=p$. Straightforward calculations show that \suppl\
=======

\vspace{-0.5cm}
\noindent
with $H_x(p)= \projp \circ \transfdet(x,p)$, $\projp(x,p)=p$. \christophe{Already used above, so should it be here?mot to Appendix} Straightforward calculations imply that \suppl\  
>>>>>>> 812d27c8fa67b85e4bad7a49278eae8d39be7436
\begin{equation}
\label{eq:NICE-identity-ratio}
\frac{q(y,x)}{q(x,y)}= \frac{\varphi(H_x(G_x^{-1}(y)))}{\varphi(G_x^{-1}(y))} \eqsp,
\end{equation}
<<<<<<< HEAD
showing that the acceptance ratio $\alpha$ defined by \eqref{eq:acceptance-NICE} is nothing more than the standard MH ratio and that  the marginal Markov kernel $P$ is $\pi_0$-reversible.

=======
% <<<<<<< HEAD
% showing that the acceptance ratio $\alpha$ defined by \eqref{eq:acceptance-NICE} is nothing more than the standard MH ratio and that  the marginal Markov kernel $K$ is $\pi_0$-reversible. We may now apply \Cref{theo:irred_and_co}
% with $\invol_0(x)=x$.
% \begin{theorem}
% Assume now that for any $k$, $M_k$ and $N_k$ are $\mathrm{L}$-Lipschitz, with $\mathrm{L}$ that also verifies, for $x$ in $\rset^d$, $\|M(x)\|\leq \mathrm{L}(1+\|x\|)$ and $\|N(x)\|\leq \mathrm{L}(1+\|x\|)$, and continuously differentiable.
% Then, we can find $h$ such that for $x_0\in\rset^d$, $\tilde{\Phi}_{x_0}$ is a $\rmc ^1$- diffeomorphism, with inverse noted $\Psi_{x_0}$, such that if $p_0\in\rset^d$, and $x_K = \tilde{\Phi}_{x_0}(p_0)$, $p_0 = \Psi_{x_0}(x_K)$.
% Moreover, the kernel
% \begin{equation}
% \bar{Q}_\alpha(x, \msa) = \int_\msa \bar{\alpha}(x, x')\varphi(\Psi_{x}(x')) \Jac_{{\Psi}_x}(x') \rmd  x'
% \end{equation}
% is irreducible, with $\bar{\alpha}(x, x') =\alpha\left\{\left(x, {\Psi}_x( x')\right), \Phi\left(x, {\Psi}_x(x')\right)\right\}$ where $\alpha$ is defined before to satisfy the $(\mu, \Sigma)$-reversibility.
% \end{theorem}
% The proof of the theorem is given in supplementary.
% =======
showing that the acceptance ratio $\alpha$ defined by \eqref{eq:acceptance-NICE} is nothing but the standard MH ratio and that  the marginal Markov kernel $K$ is $\pi_0$-reversible. 
>>>>>>> 812d27c8fa67b85e4bad7a49278eae8d39be7436

We may now apply \Cref{theo:irred_and_co}
with $\invol_0(x)=x$.



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main-t"
%%% End:

